On-Policy Model Errors in Reinforcement Learning

Model-free reinforcement learning algorithms can compute policy gradients given sampled environment transitions, but require large amounts of data. In contrast, model-based methods can use the learned model to generate new data, but model errors and bias can render learning unstable or suboptimal. In this paper, we present a novel method that combines real-world data and a learned model in order to get the best of both worlds. The core idea is to exploit the real-world data for on-policy predictions and use the learned model only to generalize to different actions. Specifically, we use the data as time-dependent on-policy correction terms on top of a learned model, to retain the ability to generate data without accumulating errors over long prediction horizons. We motivate this method theoretically and show that it counteracts an error term for model-based policy improvement. Experiments on MuJoCo- and PyBullet-benchmarks show that our method can drastically improve existing model-based approaches without introducing additional tuning parameters.

==> OPC Paper ICLR/figures/example_1d/ex_1d_gradient_errors.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.95\linewidth, trim=0 0 0 0, clip]{figures/example_1d/ex_1d_grad_error_visualization_action.png}
    \caption{Signed gradient error when using inaccurate models \cref{eq:ex1d_approx_system} to estimate the policy gradient without (left) and with (right) \ourmethod.
        The background's opacity depicts the error's magnitude, whereas color denotes if the sign of estimated and true gradient differ (red) or coincide (blue).
        \ourmethod improves the gradient estimate in the presence of model errors.
        Note that the optimal policy is $\theta^* = -1.0$.
    }
    \label{fig:ex1d_gradient_errors}
\end{figure*}

==> OPC Paper ICLR/figures/gym_results/gym_results.tex <==
\begin{figure}[t]
\centering

\begin{subfigure}[b]{.32\linewidth}
    \includegraphics[width=\linewidth]{figures/gym_results/gym_zoo_invertedpendulum.pdf}
\end{subfigure} %
\begin{subfigure}[b]{.32\linewidth}
    \includegraphics[width=\linewidth]{figures/gym_results/gym_zoo_hopper.pdf}
\end{subfigure} %
\begin{subfigure}[b]{.32\linewidth}
    \includegraphics[width=\linewidth]{figures/gym_results/gym_zoo_halfcheetah.pdf}
\end{subfigure}

\begin{tikzpicture}
  \footnotesize
  \def\barhalfheight{0.15}
  \def\barwidth{0.6}
  \def\dy{0.5}
  \def\dxtext{0.9}
  \def\dxbar{0.2}
  \def\dx{3.2}
  
  % Methods
  \newcommand{\LegendList}{
  1/tableauC0/solid/\ourmethod (ours), 
  2/tableauC1/dashed/\mbpo $\realratio = 5\%$,
  3/tableauC2/dashed/\mbpo $\realratio = 0\%$,
  4/tableauC3/dotted/\sac
  }
  
\foreach \i/\markercolor/\linestyle/\entry in \LegendList {
    \node[anchor=west] at (\dxtext + \i*\dx,0.0) {\entry};
    \fill [\markercolor!30!white] (\dxbar + \i*\dx,\barhalfheight) rectangle (\dxbar + \i*\dx + \barwidth, -\barhalfheight);
    \draw [-,\markercolor, \linestyle, line width = 1.0pt] (\dxbar + \i*\dx, 0.0) -- (\dxbar + \i*\dx + \barwidth, 0.0);
}
\end{tikzpicture}


\caption{Results based on original implementation \cref{app:evaluation_original_mbpo}: Comparison of \ourmethod to the model-based \mbpo and model-free \sac algorithms. 
The two \mbpo variants differ in terms of the mix-in ratio $\realratio$ of real off-policy transitions in the training data -- a critical hyperparameter.
All model-based approaches outperform \sac in terms of convergence for the high-dimensional tasks. 
Moreover, on the highly stochastic Hopper environment, \ourmethod outperforms both \mbpo variants and does not require additional real off-policy data.}
\label{fig:gym_results_original_implementation}
\end{figure}

==> OPC Paper ICLR/figures/large_ablation/large_ablation.tex <==
\begin{figure}
\centering

\begin{minipage}[t]{0.33\linewidth}
\includegraphics[width=\linewidth]{figures/large_ablation/hopper_ratio_0.0_length_1.pdf}
\end{minipage}\hfill
\begin{minipage}[t]{0.33\linewidth}
\includegraphics[width=\linewidth]{figures/large_ablation/hopper_ratio_0.05_length_1.pdf}
\end{minipage}\hfill
\begin{minipage}[t]{0.33\linewidth}
\includegraphics[width=\linewidth]{figures/large_ablation/hopper_ratio_0.1_length_1.pdf}
\end{minipage}

\begin{minipage}[t]{0.33\linewidth}
\includegraphics[width=\linewidth]{figures/large_ablation/hopper_ratio_0.0_length_5.pdf}
\end{minipage}\hfill
\begin{minipage}[t]{0.33\linewidth}
\includegraphics[width=\linewidth]{figures/large_ablation/hopper_ratio_0.05_length_5.pdf}
\end{minipage}\hfill
\begin{minipage}[t]{0.33\linewidth}
\includegraphics[width=\linewidth]{figures/large_ablation/hopper_ratio_0.1_length_5.pdf}
\end{minipage}

\begin{minipage}[t]{0.33\linewidth}
\includegraphics[width=\linewidth]{figures/large_ablation/hopper_ratio_0.0_length_10.pdf}
\end{minipage}\hfill
\begin{minipage}[t]{0.33\linewidth}
\includegraphics[width=\linewidth]{figures/large_ablation/hopper_ratio_0.05_length_10.pdf}
\end{minipage}\hfill
\begin{minipage}[t]{0.33\linewidth}
\includegraphics[width=\linewidth]{figures/large_ablation/hopper_ratio_0.1_length_10.pdf}
\end{minipage}

\begin{minipage}[t]{0.33\linewidth}
\includegraphics[width=\linewidth]{figures/large_ablation/hopper_ratio_0.0_length_20.pdf}
\end{minipage}\hfill
\begin{minipage}[t]{0.33\linewidth}
\includegraphics[width=\linewidth]{figures/large_ablation/hopper_ratio_0.05_length_20.pdf}
\end{minipage}\hfill
\begin{minipage}[t]{0.33\linewidth}
\includegraphics[width=\linewidth]{figures/large_ablation/hopper_ratio_0.1_length_20.pdf}
\end{minipage}

\begin{tikzpicture}
  \footnotesize
  \def\barhalfheight{0.15}
  \def\barwidth{0.6}
  \def\dy{0.5}
  \def\dxtext{0.9}
  \def\dxbar{0.2}
  \def\dx{6.0}
  
%   \pgfmathsetmacro\I{int(mod(\i,2))}

  
  % Methods
  \newcommand{\LegendList}{
  0/tableauC0/solid/\ourmethod + reset buffer, 
  1/tableauC0/dashed/\ourmethod + not reset buffer,
  2/tableauC2/solid/\mbpo + reset buffer + deterministic,
  3/tableauC2/dashed/\mbpo + not reset buffer + deterministic,
  4/tableauC3/solid/\mbpo + reset buffer + stochastic,
  5/tableauC3/dashed/\mbpo + not reset buffer + stochastic
  }
  
% \node[anchor=east] at (0.0,0.0) {Rollout length: };
\foreach \i/\markercolor/\linestyle/\entry in \LegendList {
    \pgfmathsetmacro\I{int(mod(\i,2))}
    \pgfmathsetmacro\J{int(\i / 2))}
    
    \node[anchor=west] at (\dxtext + \I*\dx, -\J * \dy) {\entry };
    \fill [\markercolor!30!white] (\dxbar + \I*\dx,\barhalfheight-\J * \dy) rectangle (\dxbar + \I*\dx + \barwidth, -\barhalfheight-\J * \dy);
    \draw [-,\markercolor, \linestyle, line width = 1.0pt] (\dxbar + \I*\dx,-\J * \dy) -- (\dxbar + \I*\dx + \barwidth, -\J * \dy);
}

\end{tikzpicture}

\caption{
Results based on original implementation \cref{app:evaluation_original_mbpo}:
Large ablation study on the Hopper environment, investigating the influence various hyperparameters and design choices.
Mix-in ratio of real data~$\realratio$ (columns): ${0\%, 5\%, 10\%}$ from left to right. 
Rollout length $\horizon$ (rows): ${1, 5, 10, 20}$ from top to bottom.
}
\label{fig:appendix_large_ablation}
\end{figure}

==> OPC Paper ICLR/figures/signed_gradient_distance/signed_gradient_distance.tex <==
\begin{figure}[htbp]
    \centering
    
\begin{tikzpicture}[
    tangent/.style={
        decoration={
            markings,% switch on markings
            mark=
                at position #1
                with
                {
                    \coordinate (tangent point-\pgfkeysvalueof{/pgf/decoration/mark info/sequence number}) at (0pt,0pt);
                    \coordinate (tangent unit vector-\pgfkeysvalueof{/pgf/decoration/mark info/sequence number}) at (1,0pt);
                    \coordinate (tangent orthogonal unit vector-\pgfkeysvalueof{/pgf/decoration/mark info/sequence number}) at (0pt,1);
                }
        },
        postaction=decorate
    },
    use tangent/.style={
        shift=(tangent point-#1),
        x=(tangent unit vector-#1),
        y=(tangent orthogonal unit vector-#1)
    },
    use tangent/.default=1
]
% \draw[step=1.0,gray,thin] (0.0,0.0) grid (6.0, 9.0);

\draw [black, thick,
    tangent=0.41,
    tangent=0.65
] (1,1)
    to [out=0,in=180] (3, 2)
    to [out=0, in=180] (5, 1);
\draw [name path=tangent 1, blue!30!white, thick, dashed, use tangent] (-1.5,0) -- (3,0);
\draw [-{Latex[length=2mm]}, blue, thick, use tangent] (0,0) -- (1.5, 0);
\node [circle, draw=blue, fill=blue, inner sep=0pt, minimum size=3pt, use tangent, label=below:{\color{blue}$g_1$}] at (0.0, 0.0) {};

\draw [name path=tangent 2, orange!30!white, thick, dashed, use tangent=2] (-2.5,0) -- (2,0);
\draw [-{Latex[length=2mm]}, orange, thick, use tangent=2] (0,0) -- (2, 0);
\node [circle, draw=orange, fill=orange, inner sep=0pt, minimum size=3pt, use tangent=2, label=below:{\color{orange}$g_2$}] at (0.0, 0.0) {};

\path [name intersections={of=tangent 1 and tangent 2,by=intersec}];
% \node [fill=red,inner sep=1pt,label=90:$E$] at (intersec) {};

\draw (intersec) ++(23:1.5) arc (23:-35:1.5) node [midway, label=right:{$\Delta g$}] {};

\end{tikzpicture}

\caption{Sketch depicting the signed gradient distance \cref{eq:signed_gradient_error}. In this particular case, gradient $g_1$ is positive and $g_2$ is negative. }
\label{fig:signed_gradient_error_sketch}
\end{figure}

==> OPC Paper ICLR/figures/state_distribution/state_distribution.tex <==
\begin{figure}
\centering
% \begin{minipage}[t]{.55\textwidth}

% timesteps
\newcommand{\tzero}{0}
\newcommand{\tone}{1}
\newcommand{\ttwo}{2}


\begin{subfigure}[b]{.49\linewidth}
    \begin{tikzpicture}
    \scriptsize

    % Debugging
    % \draw[step=1.0,gray,thin] (0.0,-1.0) grid (7.0, 4.0);

    %%%%%%%%%%%%%%%%%%%%%%%
    %%% Timestep 0 -> 1 %%%
    %%%%%%%%%%%%%%%%%%%%%%%

    % Replay buffer
    \node[circle,draw=black, fill=black, inner sep=0pt,minimum size=5pt, label=above:{$\refstate_{\tzero}^{\batch} = {\color{tableauC2} \state_0}$}] (shat0) at (0.0, 2.0) {};
    \node[circle,draw=black, fill=black, inner sep=0pt,minimum size=5pt, 
    label=left:{$\refstate_{\tone}^{\batch} = \color{black} \opcmodel( \state_{\tone} | \refstate_{\tzero}^{\batch}, \refaction_{\tzero}^\batch, \batch)$}] (shat1) at (2.5, 0.0) {};
    \draw [-{Latex[length=2mm]}, dashed] (shat0) -- (shat1);
    
    % On-policy model prediction
    \node[circle,draw=tableauC0, fill=tableauC0, inner sep=0pt,minimum size=5pt, label=below:{\color{tableauC0}$\learnedmodel(\state_{\tone} | \refstate_{\tzero}^{\batch}, \refaction^\batch_{\tzero})$}] (smean1) at (2.3, 2.0) {};
    \fill[rotate around={70:(smean1)},tableauC0, fill=tableauC0, fill opacity=0.1] (smean1) ellipse (0.4cm and 0.9cm);
    \draw [-{Latex[length=2mm]}, tableauC0] (shat0) -- (smean1);
    % \draw [-{Latex[length=2mm]}, tableauC0] (shat0) -- (smean1)
    % node[midway, below] {$\tilde{f}(\refstate_{\tzero}^{\batch}, \refaction_{\tzero}^{\batch})$};
    
    % Off-policy model prediction
    \node[circle,draw=tableauC3, fill=tableauC3, inner sep=0pt,minimum size=5pt, label=above left:{\color{tableauC3}$\learnedmodel(\state_{\tone} | \state_{\tzero}, \action_{\tzero})$}] (smodel1) at (2.5, 2.9) {};
    \fill[rotate around={80:(smodel1)},tableauC3, fill=tableauC3, fill opacity=0.1] (smodel1) ellipse (0.5cm and 1cm);
    \draw [-{Latex[length=2mm]}, tableauC3] (shat0) -- (smodel1);
    % \draw [-{Latex[length=2mm]}, tableauC3] (shat0) -- (smodel1) node[midway,sloped,above] {$\tilde{f}(\state_\tzero, \action_\tzero)$};

    % On-policy correction
    \node[circle,draw=tableauC2, fill=tableauC2, inner sep=0pt,minimum size=5pt, label=below left:{\color{tableauC2}$\opcmodel(\state_{\tone} | \state_{\tzero}, \action_{\tzero},\batch)$}] (sopc1) at (2.7, 0.9) {};
    \draw [-{Latex[length=2mm]}, tableauC2] (shat0) -- (sopc1);
    \draw [-{Latex[length=2mm]}, gray] (shat1) -- (sopc1);
    \draw [-{Latex[length=2mm]}, gray] (smean1) -- (smodel1);
    
    
    %%%%%%%%%%%%%%%%%%%%%%%
    %%% Timestep 1 -> 2 %%%
    %%%%%%%%%%%%%%%%%%%%%%%

    % Replay buffer
    \node[circle,draw=black, fill=black, inner sep=0pt,minimum size=5pt, 
    % label=right:{$\refstate_{\ttwo}^{\batch} $},
    label=above:{$\refstate_{\ttwo}^{\batch} = \color{black} \opcmodel( \state_{\ttwo} | \refstate_{\tone}^{\batch}, \refaction_{\tone}^\batch, \batch) 
        $}] (shat2) at (5.0, 2.0) {};
    \draw [-{Latex[length=2mm]}, dashed] (shat1) -- (shat2);

    % On-policy model prediction
    \node[circle,draw=tableauC0, fill=tableauC0, inner sep=0pt,minimum size=5pt, label=above left:{\color{tableauC0}$\learnedmodel(\state_{\ttwo} | \refstate_{\tone}^{\batch}, \refaction^\batch_{\tone})$}] (smean2) at (5.7, 0.2) {};
    \fill[rotate around={-70:(smean2)},tableauC0, fill=tableauC0, fill opacity=0.1] (smean2) ellipse (0.4cm and 0.9cm);
    \draw [-{Latex[length=2mm]}, tableauC0] (shat1) -- (smean2);
    % \draw [-{Latex[length=2mm]}, tableauC0] (shat1) -- (smean2)
    % node[midway, sloped, above] {$\tilde{f}(\refstate_{\tone}^{\batch}, \refaction_{\tone}^{\batch})$};

    % Off-policy model prediction
    \node[circle,draw=tableauC3, fill=tableauC3, inner sep=0pt,minimum size=5pt, label=above:{\color{tableauC3}$\learnedmodel(\state_{\ttwo} | \state_{\tone}, \action_{\tone})$}] (smodel2) at (5.5, 1.2) {};
    \fill[rotate around={-80:(smodel2)},tableauC3, fill=tableauC3, fill opacity=0.1] (smodel2) ellipse (0.5cm and 1cm);
    \draw [-{Latex[length=2mm]}, tableauC3] (sopc1) -- (smodel2);
    % \draw [-{Latex[length=2mm]}, tableauC3] (sopc1) -- (smodel2)
    % node[midway,sloped,below] {$\tilde{f}(\state_\tone, \action_\tone)$};
    
    % On-policy correction
    \node[circle,draw=tableauC2, fill=tableauC2, inner sep=0pt,minimum size=5pt, label=above:{\color{tableauC2}$\opcmodel(\state_{\ttwo} | \state_{\tone}, \action_{\tone}, \batch)$}] (sopc2) at (4.8, 3.0) {};
    \draw [-{Latex[length=2mm]}, tableauC2] (sopc1) -- (sopc2);
    \draw [-{Latex[length=2mm]}, gray] (shat2) -- (sopc2);
    \draw [-{Latex[length=2mm]}, gray] (smean2) -- (smodel2);

\end{tikzpicture}
\caption{Multi-step predictions with \ourmethod for a given $\iteration$.}
\label{fig:state_propagation}
\end{subfigure} %
\hfill
\begin{subfigure}[b]{.49\linewidth}
    % TO debug, include "frame" as an option.
    \includegraphics[scale=1]{figures/state_distribution/state_distribution_visualization2.pdf}
    \caption{State distribution over time.}
    \label{fig:state_distribution}
% \end{minipage}
\end{subfigure}
\caption{
    Illustration to compare predictions of the three models \cref{eq:replay_buffer_trajectory,eq:model_learning,eq:opc_model} starting from the same state $\refstate_\tzero^\batch$. In \cref{fig:state_propagation}, we see that on-policy, i.e., using actions $(\refaction^\batch_\tzero, \refaction^\batch_\tone)$, $\datamodel$ returns environment data, while $\learnedmodel$ (blue) is biased. We correct this on-policy bias in expectation to obtain $\opcmodel$. This allows us to retain the true state distribution when predicting with these models recursively (c.f., bottom three lines in \cref{fig:state_distribution}). 
    When using \ourmethod for off-policy actions ($\action_\tzero, \action_\tone$), $\opcmodel$ does not recover the true off-policy state distribution since it relies on the biased model.
    However, the corrections generalize locally and reduce prediction errors in \cref{fig:state_distribution} (top three lines).
}
\end{figure}



 

==> OPC Paper ICLR/figures/tikz/do_not_remove.tex <==
%

==> OPC Paper ICLR/figures_iclr/data_ablation/data_ablation.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.95\linewidth]{figures_iclr/data_ablation/data_ablation_figure.pdf}
\caption{Ablation study for \ourmethod on the HalfCheetah environment. In each plot, we fix the number of simulated transitions $N$ and vary the rollout lengths $\horizon = \{1 (\protect\saclegendentry), 5 (\protect\mbpolegendentry), 10 (\protect\opclegendentry)\}$.
% The results indicate that more diverse data improves performance.
% The results indicate that multi-step rollouts generate more diverse data, which is required for efficient learning.
}
\label{fig:data_ablation}
\end{figure}

==> OPC Paper ICLR/figures_iclr/gym_results/gym_results.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.95\linewidth]{figures_iclr/gym_results/gym_zoo_halfcheetahmujocoenv_halfcheetah_hoppermujocoenv_hopper_walker2dmujocoenv_walker2d_antmujocotruncatedobsenv_anttruncatedobs.pdf}

\caption{Comparison of 
\ourmethod (\protect\opclegendentry), \mbpoepisodic (\protect\mbpolegendentry) and \sac (\protect\saclegendentry)
on four environments from the MuJoCo control suite (top row) and their respective PyBullet implementations (bottom row). 
% While the respective performances are comparable for the MuJoCo environments, \mbpoepisodic is not able to learn successful policies for the PyBullet environments without \ourmethod.
}
\label{fig:gym_results}
\end{figure}

==> OPC Paper ICLR/figures_iclr/gym_results_ablation/gym_results_ablation.tex <==
\begin{figure}[h]
\centering
\includegraphics[width=\linewidth]{figures_iclr/gym_results_ablation/gym_zoo_halfcheetahmujocoenv_halfcheetah_hoppermujocoenv_hopper_walker2dmujocoenv_walker2d_antmujocotruncatedobsenv_anttruncatedobs.pdf}

\begin{tikzpicture}
  \footnotesize
  \def\barhalfheight{0.15}
  \def\barwidth{0.6}
  \def\dy{0.5}
  \def\dxtext{0.9}
  \def\dxbar{0.2}
  \def\dx{3.2}
  
  % Methods
  \newcommand{\LegendList}{
  1/tableauC0/solid/\ourmethod (50), 
  2/tableauC0/dotted/\ourmethod (5),
  3/tableauC3/solid/\mbpoepisodic (50),
  4/tableauC3/dotted/\mbpoepisodic (5)
  }
  
\foreach \i/\markercolor/\linestyle/\entry in \LegendList {
    \node[anchor=west] at (\dxtext + \i*\dx,0.0) {\entry};
    \fill [\markercolor!30!white] (\dxbar + \i*\dx,\barhalfheight) rectangle (\dxbar + \i*\dx + \barwidth, -\barhalfheight);
    \draw [-,\markercolor, \linestyle, line width = 1.0pt] (\dxbar + \i*\dx, 0.0) -- (\dxbar + \i*\dx + \barwidth, 0.0);
}
\end{tikzpicture}

\caption{Ablation study for 
\ourmethod and \mbpoepisodic
on four environments from the MuJoCo control suite (top row) and their respective PyBullet implementations (bottom row). We vary the \mbox{\texttt{retain epochs}} hyperparameter (indicated by the number in the parentheses behind the legend entries), i.e., the number of epochs that are kept in the data buffer for the simulated data.
}
\label{fig:gym_results_retain_epochs_ablation}
\end{figure}

==> OPC Paper ICLR/figures_iclr/mbpo_baselines/mbpo_baselines.tex <==
\begin{figure}[ht]
\centering

\begin{minipage}[t]{0.49\linewidth}
\includegraphics[width=\linewidth]{figures_iclr/mbpo_baselines/mbpo_baseline_halfcheetah.pdf}
\end{minipage}\hfill
\begin{minipage}[t]{0.49\linewidth}
\includegraphics[width=\linewidth]{figures_iclr/mbpo_baselines/mbpo_baseline_hopper.pdf}
\end{minipage}

\begin{minipage}[t]{0.49\linewidth}
\includegraphics[width=\linewidth]{figures_iclr/mbpo_baselines/mbpo_baseline_walker2d.pdf}
\end{minipage}\hfill
\begin{minipage}[t]{0.49\linewidth}
\includegraphics[width=\linewidth]{figures_iclr/mbpo_baselines/mbpo_baseline_anttruncatedobs.pdf}
\end{minipage}

\begin{tikzpicture}
  \footnotesize
  \def\barhalfheight{0.15}
  \def\barwidth{0.6}
  \def\dy{0.5}
  \def\dxtext{0.9}
  \def\dxbar{0.2}
  \def\dx{2.5}
  
% Methods
\newcommand{\LegendList}{
1/tableauC0/solid/\ourmethod, 
2/tableauC1/dashed/\mbpoepisodic,
3/tableauC1/solid/\mbpo,
4/tableauC2/solid/\textsc{pets}
}

  \newcommand{\LegendListTwo}{
  1/tableauC3/solid/\textsc{steve},
  2/tableauC4/solid/\textsc{sac}, 
  3/tableauC5/solid/\textsc{ppo},
  4/tableauC6/solid/\textsc{slbo}
  }

  
\foreach \i/\markercolor/\linestyle/\entry in \LegendList {
    \node[anchor=west] at (\dxtext + \i*\dx,0.0) {\entry};
    \fill [\markercolor!30!white] (\dxbar + \i*\dx,\barhalfheight) rectangle (\dxbar + \i*\dx + \barwidth, -\barhalfheight);
    \draw [-,\markercolor, \linestyle, line width = 1.0pt] (\dxbar + \i*\dx, 0.0) -- (\dxbar + \i*\dx + \barwidth, 0.0);
}

\foreach \i/\markercolor/\linestyle/\entry in \LegendListTwo {
    \node[anchor=west] at (\dxtext + \i*\dx,0.0 - \dy) {\entry};
    \fill [\markercolor!30!white] (\dxbar + \i*\dx,\barhalfheight - \dy) rectangle (\dxbar + \i*\dx + \barwidth, -\barhalfheight - \dy);
    \draw [-,\markercolor, \linestyle, line width = 1.0pt] (\dxbar + \i*\dx, 0.0 - \dy) -- (\dxbar + \i*\dx + \barwidth, 0.0 - \dy);
}

\end{tikzpicture}


\caption{Comparison of \ourmethod against a range of baseline methods on three MuJoCo environments. We present the mean and standard deviation across 5 independent experiments (10 for \ourmethod and \mbpoepisodic). The original data for \mbpo and the other baselines were provided by \citet{janner2019trust}. Solid lines represent the mean and the shaded areas correspond to mean $\pm$ one standard deviation.}
\label{fig:appendix_mbpo_baselines}
\end{figure}

==> OPC Paper ICLR/figures_iclr/pendulum_parameterization/pendulum_parameterization.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.95\linewidth]{figures_iclr/pendulum_parameterization/pendulum_parameterization_figure.pdf}
\caption{Comparison of \ourmethod (\protect\opclegendentry) and \mbpoepisodic (\protect\mbpolegendentry) on different variants of the CartPole environment. When the pole's angle $\vartheta$ is observed directly (center plots), both algorithms successfully learn a policy. With the sine/cosine transformations (outer plots), \mbpoepisodic fails to solve the task.}
\label{fig:pendulum_parameterization}
\end{figure}

==> OPC Paper ICLR/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

% \newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> OPC Paper ICLR/sections/experiments.tex <==
\section{Experimental Results}
\label{sec:experiments}
%
We begin the experimental section with a motivating example on a toy problem to highlight the impact of \ourmethod on the policy gradient estimates in the presence of model errors. 
The remainder of the section focuses on comparative evaluations and ablation studies on complex continuous control tasks.

\subsection{Illustrative Example} 
\label{sec:motivating_example}
%
In \cref{sec:theoretical_analysis}, we investigate the influence of the model error directly on the expected return from a theoretical perspective.
From a practical standpoint, another relevant question is how the policy optimization and the respective policy gradients are influenced by model errors.
For general environments and reward signals, this question is difficult to answer, due to the typically high-dimensional state/action spaces and large number of parameters governing the dynamics model as well as the policy.
To shed light on this open question, we resort to a simple low-dimensional example and investigate how \ourmethod improves the gradient estimates under a misspecified dynamics model.

In particular, we assume a one-dimensional deterministic environment with linear transitions and a linear policy.
The benefits of this example are that we can 1) compute the true policy gradient based on a single rollout (determinism), 2) determine the environment's closed-loop stability under the policy (linearity), and 3) visualize the gradient error as a function of all relevant parameters (low dimensionality).
The dynamics and initial state distribution are specified by $ p(\state_{\ti + 1} \mid \state_\ti, \action_\ti) = \delta(\A \state_\ti + \B \action_\ti \mid \state_\ti, \action_\ti)$ with $ \rho(\state_0) = \delta(\state_0)$
where $\A,\B \in \R$ and $\delta(\cdot)$ denotes the Dirac-delta distribution.
We define a deterministic linear policy $\pi_\theta(\action_\ti \mid \state_\ti) = \delta(\theta \state_\ti \mid \state_\ti)$ that is parameterized by the scalar $\theta \in \R$. The objective is to drive the state to zero, which we encode with an exponential reward $r(\state_\ti, \action_\ti) = \exp\left\{ -(\state_\ti / \sigma_r)^2 \right\}$.
Further, we assume an approximate dynamics model 
\begin{align}
\label{eq:ex1d_approx_system}
    \tilde{p}(\state_{\ti + 1} \mid \state_\ti, \action_\ti) = \delta((\A + \Delta \A) \state_\ti + (\B + \Delta \B) \action_\ti \mid \state_\ti, \action_\ti),
\end{align}
where $\Delta \A, \Delta \B$ quantify the mismatch between the approximate model and the true environment.
In practice, the mismatch can arise due to noise-corrupted observations of the true state or, in the case of stochastic environments, due to a finite amount of training data.

\input{figures/example_1d/ex_1d_gradient_errors}

With the setting outlined above, we investigate how model errors influence the estimation of policy gradients.
To this end, we roll out different policies under models with varying degrees of error $\Delta \B$.
For each policy/model combination, we compute the model-based policy gradient and compare it to the true gradient.
The results are summarized in \cref{fig:ex1d_gradient_errors}, where the background's opacity depicts the gradient error's magnitude and its color indicates whether the respective signs of the gradients are the same (blue, $\geq0$) or differ (red, $<0$).
For policy optimization, the sign of the gradient estimate is paramount.
However, we see in the left-hand image that even small model errors can lead to the wrong sign of the gradient.
\ourmethod significantly reduces the magnitude of the gradient error and increases the robustness towards model errors.
See also \cref{app:motivating_example} for a more in-depth analysis. % of the example.
% The definition of the signed gradient error and a more in-depth analysis of this example are presented in \cref{app:motivating_example}.

\subsection{Evaluation on Continuous Control Tasks}
\label{sec:exp_continuous_control}
%
In the following section, we investigate the impact of \ourmethod on a range of continuous control tasks.
To this end, we build upon the current state-of-the-art model-based \gls{rl} algorithm \mbpo \citep{janner2019trust}.
Further, we aim to answer the important question about how data diversity affects \gls{mbrl}, and \ourmethod in particular.
While having a model that can generate (theoretically) an infinite amount of data is intriguing, the benefit of having more data is limited by the model quality in terms of being representative of the true environment.
For \ourmethod, the following questions arise from this consideration:
Do longer rollouts help to generate better data? And is there a limit to the value of simulated transition data, i.e., is more always better?

For the dynamics model $\learnedmodel$, we follow \citet{Chua2018pets,janner2019trust} and use a probabilistic ensemble of neural networks, where each head predicts a Gaussian distribution over the next state and reward. 
For policy optimization, we employ the soft actor critic (\sac) algorithm by \citet{Haarnoja2018SoftActorCritic}.
All learning curves are presented in terms of the median (lines) and interquartile range (shaded region) across ten independent experiments, where we smooth the evaluation return with a moving average filter to accentuate the results of particularly noisy environments.
Apart from small variations in the hyperparameters, the only difference between \ourmethod and \mbpo is that our method uses $\opcmodel$, while \mbpo uses $\learnedmodel$. We provide pseudo-code for the model rollouts of \mbpo and \ourmethod in \cref{alg:opc_rollouts} in \cref{app:opc_rollouts}.
Generally, we found that \ourmethod was more robust to the choice of hyperparameters.
The rollout horizon to generate training data is set to $\horizon=10$ for all experiments.
% An overview of all relevant hyperparameters is provided in \cref{app:hyperparameters}.
Note that when using $\datamodel$ to generate data, we retain the standard (model-free) \sac algorithm.

\input{figures_iclr/gym_results/gym_results}

Our implementation is based upon the code from \citet{janner2019trust}.
We made the following changes to the original implementation: 
1) The policy is only updated at the end of an epoch, not during rollouts on the true environment.
2) The replay buffer retains data for a fixed number of episodes, to clearly distinguish on- and off-policy data.
3) For policy optimization, \mbpo uses a small number of environment transitions in addition to those from the model. We found that this design choice did not consistently improve performance and added another level of complexity. Therefore, we refrain from mixing environment and model transitions and only use simulated data for policy optimization.
While we stay true to the key ideas of \mbpo under these changes, we denote our variant as \mbpoepisodic to avoid ambiguity.
See \cref{app:mbpo_changes,app:evaluation_original_mbpo} for a comparison to the original \mbpo algorithm.
% A more detailed comparison to the original \mbpo algorithm is provided in \cref{app:mbpo_changes,app:evaluation_original_mbpo}.

\input{figures_iclr/pendulum_parameterization/pendulum_parameterization}
\paragraph{Comparative Evaluation}
%
We begin our analysis with a comparison of our method to \mbpoepisodic and \sac on four continuous control benchmark tasks from the MuJoCo control suite \citep{todorov2012mujoco} and their respective PyBullet variants \citep{benelot2018pybulletgym}.
The results are presented in \cref{fig:gym_results}.
We see that the difference in performance between both methods is only marginal when evaluated on the MuJoCo environments (\cref{fig:gym_results}, top row).
Notably, the situation changes drastically for the PyBullet environments (\cref{fig:gym_results}, bottom row).
Here, \mbpoepisodic exhibits little to no learning progress, whereas \ourmethod succeeds at learning a good policy with few interactions in the environment.
One of the main differences between the environments (apart from the physics engine itself) is that the PyBullet variants have initial state distributions with significantly larger variance.

\paragraph{Influence of State Representation}
%
In general, the success of \gls{rl} algorithms should be agnostic to the way an environment represents its state.
In robotics, joint angles $\vartheta$ are often re-parameterized by a sine/cosine transformation, $\vartheta \mapsto [\sin(\vartheta), \cos(\vartheta)]$.
We show that even for the simple CartPole environment, the parameterization of the pole's angle has a large influence on the performance of \gls{mbrl}.
In particular, we compare \ourmethod and \mbpoepisodic on the RoboSchool and PyBullet variants of the CartPole environment, which represent the pole's angle with and without the sine/cosine transformation.
The results are shown in \cref{fig:pendulum_parameterization}.
To rule out other effects than the angle's representation, we repeat the experiment for each implementation but transform the state to the other representation, respectively.
Notably, \ourmethod successfully learns a policy irrespective of the state's representation, whereas \mbpoepisodic fails if the angle of the pole is represented by the sine/cosine transformation.

\paragraph{Influence of Data Diversity}
%
Here, we investigate whether multi-step predictions are in fact beneficial compared to single-step predictions during the data generation process.
To this end, we keep the total number of simulated transitions $N$ for training constant, but choose different horizon lengths $H = \{1, 5, 10\}$.
The corresponding numbers of simulated rollouts are then given by $n_{\text{rollout}} = N / H$.
The results for $N = \{20 , 40 , 100 , 200\} \times 10^3$ on the HalfCheetah environment are shown in \cref{fig:data_ablation}.
First, note that more data leads to a higher asymptotic return, but after a certain point more data only leads to diminishing returns.
Further, the results indicate that one-step predictions are not enough to generate sufficiently diverse data.
% , but instead multi-step rollouts are in fact required.
Note that this result contradicts the findings by \citet{janner2019trust} that one-step predictions are often sufficient for \mbpo.
\input{figures_iclr/data_ablation/data_ablation}


==> OPC Paper ICLR/sections/intro.tex <==
\section{Introduction}
%
Model-free \gls{rl} has made great advancements in diverse domains such as single- and multi-agent game playing \citep{mnih2015human,silver2016alphago,vinyals2019grandmaster}, robotics \citep{kalashnikov2018qtopt}, and neural architecture search \citep{zoph2016nasrl}. All of these model-free approaches rely on large numbers of interactions with the environment to ensure successful learning.
While this issue is less severe for environments that can easily be simulated, it limits the applicability of model-free \gls{rl} to (real-world) domains where data is scarce.

\Gls{mbrl} reduces the amount of data required for policy optimization by approximating the environment with a learned model, which we can use to generate simulated state transitions \citep{Sutton1990Dyna,racaniere2017imagination,moerland2020mbrlsurvey}.
While early approaches on low-dimensional tasks by \citet{schneider1997exploiting,Deisenroth2011PILCO} used probabilistic models with closed-form posteriors, recent methods rely on neural networks to scale to complex tasks on discrete \citep{kaiser2019modelatari} and continuous \citep{Chua2018pets, kurutach2018metrpo} action spaces.
However, the learned representation of the true environment always remains imperfect, which introduces approximation errors to the \gls{rl} problem  \citep{atkeson1997comparison,abbeel2006inaccuratemodels}.
Hence, a key challenge in \gls{mbrl} is \textit{model-bias}; small errors in the learned models that compound over multi-step predictions and lead to lower asymptotic performance than model-free methods. 

To address these challenges with both model-free and model-based \gls{rl}, \citet{levine2013guided,chebotar2017combining} propose to combine the merits of both.
While there are multiple possibilities to combine the two methodologies, in this work we focus on improving the model's predictive state distribution such that it more closely resembles the data distribution of the true environment.

\paragraph{Contributions}
The main contribution of this paper is on-policy corrections (\ourmethod), a novel hyperparameter-free methodology that uses on-policy transition data on top of a separately learned model to enable accurate long-term predictions for \gls{mbrl}. A key strength of our approach is that it does not introduce any new parameters that need to be hand-tuned for specific tasks.
We theoretically motivate our approach by means of a policy improvement bound and show that we can recover the true state distribution when generating trajectories on-policy with the model.
We illustrate how \ourmethod improves the quality of policy gradient estimates in a simple toy example and evaluate it on various continuous control tasks from the MuJoCo control suite and their PyBullet variants. There, we demonstrate that \ourmethod improves current state-of-the-art \gls{mbrl} algorithms in terms of data-efficiency, especially for the more difficult PyBullet environments.

\paragraph{Related Work}
%
To counteract model-bias, several approaches combine ideas from model-free and model-based \gls{rl}. 
For example, \citet{levine2013guided} guide a model-free algorithm via model-based planning towards promising regions in the state space, \citet{kalweit2017uncertainty} augment the training data by an adaptive ratio of simulated transitions, \citet{talvitie2017self} use `hallucinated' transition tuples from simulated to observed states to self-correct the model, and \citet{feinberg2018mbve,buckman2018steve} use a learned model to improve the value function estimate.
\citet{janner2019trust} mitigate the issue of compounding errors for long-term predictions by simulating short trajectories that start from real states. 
% \citet{janner2019trust} use the learned model only for short simulated rollouts starting from real observed states to mitigate the issue of compounding errors for long-term predictions.
\citet{cheng2019predictor} extend first-order model-free algorithms via adversarial online learning to leverage prediction models in a regret-optimal manner.
% Instead of adding simulated transitions to the training data,
\citet{clavera2020maac} employ a model to augment an actor-critic objective and adapt the planning horizon to interpolate between a purely model-based and a model-free approach.
\citet{Morgan2021ModelPredictiveActorCritic} combine actor-critic methods with model-predictive rollouts to guarantee near-optimal simulated data and retain exploration on the real environment.
A downside of most existing approaches is that they introduce additional hyperparameters that are critical to the learning performance \citep{zhang21hyperparameters}.

In addition to empirical performance, recent work builds on the theoretical guarantees for model-free approaches by \citet{Kakade02approximatelyoptimal,schulman2015trust} to provide guarantees for \gls{mbrl}.
\citet{luo2018slbo} provide a general framework to show monotonic improvement towards a local optimum of the value function, while  \citet{janner2019trust} present a lower-bound on performance for different rollout schemes and horizon lengths. \citet{yu2020mopo} show guaranteed improvement in the offline \gls{mbrl} setting by augmenting the reward with an uncertainty penalty, while \citet{clavera2020maac} present improvement guarantees in terms of the model's and value function's gradient errors.

Moreover, \citet{harutyunyan2016q} propose a similar correction term as the one introduced in this paper in the context of off-policy policy evaluation and correct the state-action value function instead of the transition dynamics.
Similarly, \citet{fonteneau2013batch} consider the problem of off-policy policy evaluation but in the batch \gls{rl} setting and propose to generate `artificial' trajectories from observed transitions instead of using an explicit model for the dynamics.

A related field to \gls{mbrl} that also combines models with data is \gls{ilc} \citep{bristow2006ilcsurvey}. While \gls{rl} typically focuses on finding parametric feedback policies for general reward functions, \gls{ilc} instead seeks an open-loop sequence of actions with fixed length to improve state tracking performance.
Moreover, the model in \gls{ilc} is often derived from first principles and then kept fixed, whereas in \gls{mbrl} the model is continuously improved upon observing new data.
The method most closely related to \gls{rl} and our approach is optimization-based \gls{ilc} \citep{owens2005iterative, schoellig2009optimization}, in which a linear dynamics model is used to guide the search for optimal actions.
Recently, \citet{Baumgaertner2020NonlinearILC} extended the \gls{ilc} setting to nonlinear dynamics and more general reward signals.
Little work is available that draws connections between \gls{rl} and \gls{ilc} \citep{zhang2019preliminary} with one notable exception:
\citet{abbeel2006inaccuratemodels} use the observed data from the last rollout to account for a mismatch in the dynamics model.
The limitations of this approach are that deterministic dynamics are assumed, the policy optimization itself requires a line search procedure with rollouts on the true environment and that it was not combined with model learning.
We build on this idea and extend it to the stochastic setting of \gls{mbrl} by making use of recent advances in \gls{rl} and model learning.

\section{Problem Statement and Background}

We consider the \gls{mdp} $(\statespace, \actionspace, p, r, \gamma, \rho)$, where $\statespace \subseteq \R^\nstate$ and $\actionspace \subseteq \R^\naction$ are the continuous state and action spaces, respectively.
The unknown environment dynamics are described by the transition probability $p(\state_{\ti + 1} \mid \state_\ti, \action_\ti)$, an initial state distribution $\rho(\state_0)$ and the reward signal $r(\state, \action)$.
The goal in \gls{rl} is to find a policy $\pi_\theta(\action_\ti \mid \state_\ti)$ parameterized by $\theta$ that maximizes the expected return discounted by $\gamma \in [0, 1]$ over episodes of length $T$,
%
\begin{align}\label{eq:rl_problem}
    \return{} = \E_{\state_{0:T}, \action_{0:T} } 
     \left[ \sum\nolimits_{\ti=0}^\Ti \gamma^\ti r(\state_\ti, \action_\ti) \right], 
    \quad
    \state_{\ti + 1} \sim p(\state_{\ti + 1} \mid \state_\ti, \action_\ti),
    \quad
    \state_0 \sim \rho,
    \quad 
    \action_\ti \sim \pi_\theta(\action_\ti \mid \state_\ti).
\end{align}
%
The expectation is taken with respect to the trajectory under the stochastic policy $\pi_\theta$ starting from a stochastic initial state $\state_0$. Direct maximization of \cref{eq:rl_problem} is challenging, since we do not know the environment's transition model $p$.
In \gls{mbrl}, we learn a model for the transitions and reward function from data, $\tilde{p}(\state_{\ti + 1} \mid \state_\ti, \action_\ti) \approx p(\state_{\ti + 1} \mid \state_\ti, \action_\ti)$ and $\tilde{r}(\state_\ti, \action_\ti) \approx r(\state_\ti, \action_\ti)$, respectively.
Subsequently, we maximize the model-based expected return $\modelreturn{}$ as a surrogate problem for the true \gls{rl} setting, where $\modelreturn{}$ is defined as in \cref{eq:rl_problem} but with $\tilde{p}$ and $\tilde{r}$ instead.
%
% , and subsequently maximize
% %
% \begin{equation}
%     \label{eq:mbrl_problem}
%     \modelreturn{} = \E_{\state_{0:T}, \action_{0:T} } \left[ \sum\nolimits_{\ti=0}^\Ti \gamma^\ti \tilde{r}(\state_\ti, \action_\ti) \right], 
%     \quad
%     \state_{\ti + 1} \sim \tilde{p}(\state_{\ti + 1} \mid \state_\ti, \action_\ti),
%     \quad
%     \state_0 \sim \tilde{\rho},
%     \quad 
%     \action_\ti \sim \pi_\theta(\action_\ti \mid \state_\ti).
% \end{equation}
% %
% as a surrogate problem for \cref{eq:rl_problem}.
% The choice of initial state distribution $\tilde{\rho}(\state_0)$ depends on the optimization method:
% For model predictive control, \citet{Chua2018pets} use the current state to optimize the next action based on a rollout, while \citet{janner2019trust} use the empirical state distribution observed from the true environment. 
% In the following, we focus on the latter and 
For ease of exposition, we assume a known reward function $\tilde{r} = r$, even though we learn it jointly with $\tilde{p}$ in our experiments.

We let $\eta_\iteration$ denote the return under the policy $\pi_\iteration = \pi_{\theta_\iteration}$ at iteration $\iteration$ and use $\refstate$ and $\refaction$ for states and actions that are observed on the true environment.
\Cref{alg:main} summarizes the overall procedure for \gls{mbrl}: At each iteration $\iteration$ we store $\batchsize$ on-policy trajectories $\data_\iteration^\batch = \{ ( \refstate^{\iteration,\batch}_{\ti}, \refaction^{\iteration,\batch}_\ti, \refstate^{\iteration,\batch}_{\ti+1} ) \}_{\ti=0}^{\Ti - 1}$ obtained by rolling out the current policy $\pi_\iteration$ on the real environment in \cref{alg:mbrl:rollout}. Afterwards, we approximate the environment with a learned model $\tilde{p}_\iteration(\state_{\ti + 1} \mid \state_\ti, \action_\ti)$ based on the data $\data_{1:n}$ in \cref{alg:mbrl:model_learning}, and optimize the policy based on the proxy objective $\modelreturn{}$ in \cref{alg:mbrl:policy_improvement}. Note that the policy optimization algorithm can be off-policy and employ its own, separate replay buffer.

\paragraph{Model Choices}
%
The choice of model $\tilde{p}$ plays a key role, since it is used to predict sequences $\tau$ of states transitions and thus defines the surrogate problem in \gls{mbrl}.
% Inside the optimization loop, the model is typically used to predict sequences $\tau$ of state transitions.
We assume that the model comes from a distribution family $\mathcal{P}$, which for each state-action pair $(\state_\ti, \action_\ti)$ models a distribution over the next state $\state_{\ti + 1}$. The model is then trained to summarize all past data $\data_{1:\iteration} = \cup_{i = 1}^{\iteration} \cup_{\batch=1}^\batchsize \data^\batch_i$ by maximizing the marginal log-likelihood $\mathcal{L}$,
%
\begin{equation}
    \label{eq:model_learning}
    \learnedmodel_\iteration(\state_{\ti + 1} \mid \state_\ti, \action_\ti) 
    = \argmax_{\tilde{p} \in \mathcal{P}} \sum_{(\refstate_\ti, \refaction_\ti, \refstate_{\ti+1}) \in \data_{1:\iteration} } \mathcal{L}(\refstate_{\ti+1}; \refstate_\ti, \refaction_\ti ).
\end{equation}
%
For a sampled trajectory index $\batch \sim
\mathcal{U}(\{1, \dots, \batchsize\})$,
% \operatorname{Categorical}( \{ 1, \dots, \batchsize \} )$,
% under this one-step model
sequences $\tau$ start from the initial state $\refstate_0^{\iteration,\batch}$ and are distributed according to $\learnedmodel_\iteration(\tau \mid \batch) = \delta(\state_0 - \refstate_0^{n,b}) \prod_{\ti=0}^{\Ti-1} \learnedmodel_\iteration(\state_{\ti+1} \mid \state_\ti, \action_\ti) \pi_\theta(\action_\ti \mid \state_\ti)$,
where $\delta(\cdot)$ denotes the Dirac-delta distribution. 
%
Using model-data for policy optimization is in contrast to model-free methods, which only use observed environment data by replaying past transitions from a recent on-policy trajectory $\batch \in \{ 1, \dots, \batchsize\}$. In our model-based framework, this replay buffer is equivalent to the non-parametric model
%
\begin{equation}
\label{eq:replay_buffer_trajectory}
     \datamodel_\iteration(\tau \mid \batch) = \delta(\state_0 - \refstate_0^{n,b}) \prod_{\ti=0}^{\Ti-1} \datamodel_\iteration(\state_{\ti+1} \mid \ti, \batch),  
     \text{~where~}
     \datamodel_\iteration(\state_{\ti+1} \mid \ti, \batch) =  \delta(\state_{\ti+1} - \refstate_{\ti+1}^{\iteration,\batch}) ,
\end{equation}
%
where we only replay observed transitions instead of sampling new actions from $\pi_\theta$.

% This model choice effectively reduces model-based algorithms back to the model-free setting.
% An alternative is 

% While we focus on $\Ti$-step rollouts starting from the empirical initial state distribution in the exposition, our methodology extends to branched rollouts \citep{janner2019trust} and model predictive control \citep{Chua2018pets}.
% The choice of the initial state depends on the optimization method:
% For model predictive control, \citet{Chua2018pets} use the current state to optimize the next action based on a rollout, while \citet{janner2019trust} sample initial states from the empirical state distribution observed on the true environment. 
% \lf{with this notation, we don't need conditioning on $\batch$ for $\learnedmodel$ trajectory distribution}
% \fb{Should we focus only on empirical initial distribution and mention the other options after theorem 1?}

% For both models, we can sample $\horizon$-step predictions by first sampling a trajectory index $\batch \sim \operatorname{Categorical}( \{ 0, \dots, \batchsize \} )$ and then rolling out following the respective state sequence distributions $\tilde{p}(\tau_{\ti:\ti+\horizon} \mid \ti, \batch)$.

\begin{algorithm}[t]
  \caption{General Model-based Reinforcement Learning}
  \label{alg:main}
  \begin{algorithmic}[1] % The number tells where the line numbering should start
    \For{$\iteration = 1,\dots$}
      \For{$\batch = 1, \dots, \batchsize$}
          \State Rollout policy $\pi_{\iteration}$ on environment and store transitions $\data_\iteration^\batch = \{ ( \refstate^{\iteration,\batch}_{\ti}, \refaction^{\iteration,\batch}_\ti, \refstate^{\iteration,\batch}_{\ti+1} ) \}_{\ti=0}^{\Ti - 1}$ 
          \label{alg:mbrl:rollout}
      \EndFor
      \State $\tilde{p}_n(\state_{\ti + 1} \mid \state_\ti, \action_\ti)$: Learn a global dynamics model given all data $\data_{1:n} = \bigcup_{i=1}^{\iteration} \bigcup_{\batch=1}^\batchsize \data_i^b $
      \label{alg:mbrl:model_learning}
      \State $\theta_{\iteration + 1} = \theta_\iteration + \alpha \nabla \modelreturn{\iteration}$: Optimize the policy based on the model $\tilde{p}$ with any \gls{rl} algorithm
      \label{alg:mbrl:policy_improvement}
    \EndFor
  \end{algorithmic}
  \label{alg:mbrl}
\end{algorithm}


==> OPC Paper ICLR/sections/main.tex <==

\section{On-policy Corrections}
\label{sec:on_policy_corrections}

In this section, we analyze how the choice of model impacts policy improvement, develop \ourmethod as a model that can eliminate one term in the improvement bound, and analyze its properties. In the following, we drop the $\iteration$ sub- and superscript when the iteration is clear from context.

\subsection{Policy Improvement}
%
Independent of whether we use the data directly in \datamodel or summarize it in a world model \learnedmodel, our goal is to find an optimal policy that maximizes \cref{eq:rl_problem} via the corresponding model-based proxy objective.
To this end, we would like to know how a policy improvement $\modelreturn{\iteration + 1} - \tilde{\eta}_\iteration \geq 0$ based on the model $\tilde{p}$, which is what we optimize in \gls{mbrl}, relates to the true gain in performance $\return{\iteration + 1} - \eta_\iteration$ on the environment with unknown transitions $p$.
While the two are equal without model errors,
% , $\tilde{p} = p$,
in general the larger the model error, the worse we expect the proxy objective to be \citep{Lambert20ObjectiveMismatch}.
Specifically, we show in \cref{ap:policy_improvement_bound} that the policy improvement can be decomposed as
%
\begin{align}\label{eq:improvement_bound}
    \undertext{True policy improvement}{
        \return{\iteration+1} - \return{\iteration}
    }
     & \geq
    \undertext{Model policy improvement}{
        \modelreturn{\iteration+1} - \modelreturn{\iteration}
    }
    - \quad
    \undertext{Off-policy model error}{
        | \return{\iteration+1} - \modelreturn{\iteration+1} |
    }
    \quad-
    \undertext{On-policy model error}{
        | \return{\iteration} - \modelreturn{\iteration} |
    }
    \, ,
\end{align}
%
where a performance improvement on our model-based objective $\modelreturn{}$ only translates to a gain in \cref{eq:rl_problem} if two error terms are sufficiently small. These terms depend on how well the performance estimate based on our model, $\modelreturn{}$, matches the true performance, $\eta$. If the reward function is known, this term only depends on the model quality of $\tilde{p}$ relative to $p$. Note that in contrast to the result by \citet{janner2019trust}, \cref{eq:improvement_bound} is a bound on the policy improvement instead of a lower bound on $\eta_{\iteration+1}$.

The first error term compares $\return{\iteration + 1}$ and $\modelreturn{\iteration + 1}$, the performance estimation gap under the optimized policy $\pi_{\iteration + 1}$ that we obtain in \cref{alg:mbrl:policy_improvement} of \cref{alg:mbrl}. Since at this point we have only collected data with $\pi_\iteration$ in \cref{alg:mbrl:rollout}, this term depends on the generalization properties of our model to new data; what we call the \emph{off-policy model error}. For our data-based model \datamodel that just replays data under $\pi_\iteration$ independently of the action, this term can be bounded for stochastic policies. For example, \citet{schulman2015trust} bound it by the average KL-divergence between $\pi_\iteration$ and $\pi_{\iteration + 1}$. For learned models \learnedmodel, it depends on the generalization properties of the model \citep{luo2018slbo,yu2020mopo}. While understanding model generalization better is an interesting research direction, we will assume that our learned model is able to generalize to new actions in the following sections.

While the first term hinges on model-generalization, the second term is the \emph{on-policy model error}, i.e., the deviation between \return{\iteration} and \modelreturn{\iteration} under the current policy $\pi_\iteration$.
This error term goes to zero for \datamodel as we use more on-policy data $\batchsize \to \infty$, since the transition data are sampled from the true environment, c.f.,
% \cref{lem:infinite_data_return} in the appendix.
\cref{ap:prop_data_model}.
While the learned model is also trained with on-policy data, small errors in our model compound as we iteratively predict ahead in time. Consequently, 
% for prediction horizons $\horizon$ shorter than the effective horizon encoded in the discount factor, $\horizon < \gamma / (1 - \gamma)$, 
the on-policy error term grows as $\bigO( \min( \gamma / (1 - \gamma)^2, \horizon / (1 - \gamma), \horizon^2 ) )$, c.f., \citep{janner2019trust} and \cref{ap:prop_learned_model}. %The root cause is the same as in behavior cloning \citep[Theorem 2.1]{ross2010efficient}, where small errors aggregate over time.


\subsection{Combining Learned Models and Replay Buffer}
\label{sec:combining_models}

The key insight of this paper is that the learned model in \cref{eq:model_learning} and the replay buffer in \cref{eq:replay_buffer_trajectory} have opposing strengths:
The replay buffer has low error on-policy, but high error off-policy since it replays transitions from past data, i.e., they are independent of the actions chosen under the new policy.
In contrast, the learned model can generalize to new actions by extrapolating from the data and thus has lower error off-policy, but errors compound over multi-step predictions.

An ideal model would combine the model-free and model-based approaches in a way such that it retains the unbiasedness of on-policy generated data, but also generalizes to new policies via the model.
To this end, we propose to use the model to predict how observed transitions would \textit{change} for a new state-action pair.
%adjust the observed transitions by an offset that accounts for the model predictions given a new state-action pair.
In particular, we use the model's mean prediction
$\tilde{f}_\iteration(\state, \action) = \E [
        \learnedmodel_\iteration( \, \cdot \mid \state, \action)
    ] $
to construct the joint model
%
\begin{align}\label{eq:opc_model}
    \opcmodel_\iteration(\state_{\ti + 1} \mid \state_\ti, \action_\ti, \batch)
     & = \undertext{$\datamodel_\iteration(\state_{\ti + 1} \mid \ti, \batch)$}{
        \delta\big(\state_{\ti+1} - \refstate^{\iteration,\batch}_{\ti+1} \big)
    }
    * \,\,\,
    \undertext{Model mean correction to generalize to $\state_\ti$, $\action_\ti$}{
        \delta\big( \state_{\ti + 1} - \big[ \tilde{f}_\iteration(\state_\ti, \action_\ti)  - \tilde{f}_\iteration(\refstate^{\iteration,\batch}_\ti, \refaction^{\iteration,\batch}_\ti ) \big] \big),
    }
\end{align}
%
where $*$ denotes the convolution of the two distributions and $\batch$ refers to a specific rollout stored in the replay buffer that was observed in the true environment. Given a trajectory-index $\batch$, $\opcmodel_\iteration$ in \cref{eq:opc_model} transitions deterministically according to $\state_{\ti + 1} = \refstate^{\iteration,\batch}_{\ti+1} + \tilde{f}_\iteration(\state_\ti, \action_\ti) - \tilde{f}_\iteration(\refstate^{\iteration,\batch}_\ti, \refaction^{\iteration,\batch}_\ti)$, resembling the equations in \gls{ilc} (c.f., \citet{Baumgaertner2020NonlinearILC} and \cref{app:connection_rl_ilc}). If we roll out $\opcmodel_\iteration$ along a trajectory, starting from a state $\refstate_\ti^{\iteration,\batch}$ and apply the recorded actions from the replay buffer, $\refaction_\ti^{\iteration,\batch}$, the correction term on the right of \cref{eq:opc_model} cancels out and we have $\opcmodel_\iteration(\state_{\ti + 1} \mid \refstate^{\iteration,\batch}_\ti, \refaction^{\iteration,\batch}_\ti, \batch) = \datamodel_\iteration(\state_{\ti + 1} \mid \ti, \batch) = \delta(\state_{\ti + 1} - \refstate^{\iteration,\batch}_{\ti + 1})$. Thus \ourmethod retrieves the true on-policy data distribution independent of the prediction quality of the model, which is why we refer to this method as \emph{on-policy corrections}~(\ourmethod). This behavior is illustrated in \cref{fig:state_propagation}, where the model (blue) is biased on-policy, but \ourmethod corrects the model's prediction to match the true data. In \cref{fig:state_distribution}, we show how this affects predicted rollouts on a simple stochastic double-integrator environment. Although small on-policy errors in \learnedmodel (blue) compound over time, the corresponding \opcmodel matches the ground-truth environment data closely. Note that even though the model in \cref{eq:opc_model} is deterministic, we retain the environment's stochasticity from the data in the transitions to $\refstate_{\ti+1}$, so that we recover the on-policy aleatoric uncertainty (noise) from sampling different reference trajectories via indexes~$\batch$.


\input{figures/state_distribution/state_distribution}

When our actions $\action_\ti$ are different from $\refaction^{\batch}_\ti$, \opcmodel still uses the data from the environment's transitions, but the correction term in \cref{eq:opc_model} uses the learned model to predict how the next state \emph{changes} in expectation relative to the prediction under $\refaction^{\batch}_\ti$. That is, in \cref{fig:state_propagation} for a new $\action_\ti$ the model predicts the state distribution shown in red. Correspondingly, we shift the static prediction $\refstate_{\ti + 1}^{\batch}$ by the difference in means (gray arrow) between the two predictions; i.e., the \emph{change in trajectory} by changing from $\refaction_\ti^{\batch}$ to $\action_\ti$. Since we shift the model predictions by a time-dependent but constant offset, this does not recover the true state distribution unless the model has zero error. However, empirically it can still help with long-term predictions in \cref{fig:state_distribution} by shifting the model off-policy predictions (red) to the \ourmethod predictions (green), which are closer to the environment's state distribution under the new policy.

\subsection{Theoretical Analysis}
\label{sec:theoretical_analysis}

In the previous sections, we have introduced \ourmethod to decrease the on-policy model error in~\cref{eq:improvement_bound} and tighten the improvement bound.
In this section, we analyze the on-policy performance gap from a theoretical perspective and show that with \ourmethod this error can be reduced independently of the learned model's error.
To this end, we assume infinitely many on-policy reference trajectories, $\batchsize \to \infty$, which is equivalent to a variant of $\opcmodel$ that considers $\refstate_{\ti+1}^{\batch}$ as a random variable that follows the true environment's transition dynamics. While impossible to implement in practice, this formulation is useful to understand our method.
%this formulation helps in the theoretical analysis.
We define the generalized \ourmethod-model as
% The generalized \ourmethod-model is defined as
%
\begin{align}
\label{eq:generalized_opc_model}
    \opcintmodel(\state_{\ti+1} \mid \state_\ti, \action_\ti, \batch) = \undertext{Environment on-policy transition}{\vphantom{\Big(}
            p( \refstate_{\ti+1} \mid \refstate_\ti^\batch, \refaction_\ti^\batch)
        }
        *\quad \undertext{\ourmethod correction term}{
            \delta \Big( \state_{\ti + 1} - \Big[ \tilde{f}(\state_\ti, \action_\ti) - \tilde{f}(\refstate_\ti^\batch, \refaction_\ti^\batch ) \Big] \Big)
        },
\end{align}
%
which highlights that it transitions according to the true on-policy dynamics conditioned on data from the replay buffer, combined with a correction term. We provide a detailed derivation for the generalized model in \cref{app:proofs}, \cref{lem:opc_distribution_general}.
With \cref{eq:generalized_opc_model}, we have the following result:

\begin{restatable}{theorem}{onpolicyerrorbound}
\label{thm:on_policy_error_bound_full}
Let $\opcreturn$ and $\return{}$ be the expected return under the generalized \ourmethod-model \cref{eq:generalized_opc_model} and the true environment, respectively.
Assume that the learned model's mean transition function $\tilde{f}(\state_\ti, \action_\ti) = \E[\learnedmodel(\state_{\ti+1} \mid \state_\ti, \action_\ti)]$ is $L_f$-Lipschitz and the reward $r(\state_\ti, \action_\ti)$ is $L_r$-Lipschitz. Further, if the policy $\pi(\action_\ti \mid \state_\ti)$ is $L_{\pi}$-Lipschitz with respect to $\state_\ti$ under the Wasserstein distance and its (co-)variance $\var[\pi(\action_\ti \mid \state_\ti)] = \Sigma_\pi(\state_\ti) \in \mathbb{S}_+^{\nact}$ is finite over the complete state space, i.e., $\max_{\state_\ti \in \statespace} \trace \{ \Sigma_\pi(\state_\ti) \} \leq \bar{\sigma}^2_\pi$, then with $C_1 = \sqrt{2 (1 + L_\pi^2)} L_f L_r$ and $C_2 = \sqrt{L_f^2 + L_\pi^2}$
%
\begin{align}
\label{eq:on_policy_error_bound_full}
    | \return{} - \opcreturn | &\leq \frac{\bar{\sigma}_\pi}{1 - \gamma}  \nact^{\frac{1}{4}} C_1  C_2^{\Ti} \sqrt{\Ti} .
\end{align}
\end{restatable}
%
We provide a proof in \cref{app:proofs_opc}.
From \cref{thm:on_policy_error_bound_full}, we can observe the key property of \ourmethod: 
for deterministic policies, the on-policy model error from \cref{eq:improvement_bound} is zero and independent of the learned models' predictive distribution \learnedmodel, so that $\return{} = \opcreturn$.
For policies with non-zero variance, the bound scales exponentially with $\Ti$, highlighting the problem of compounding errors. In this case, as in the off-policy case, the model quality determines how well we can generalize to different actions. We show in \cref{ap:opc_model_error_analysis} that, for one-step predictions, \ourmethod's prediction error scales as the minimum of policy variance and model error. To further alleviate the issue of compounding errors, one could extend \cref{thm:on_policy_error_bound_full} with a branched rollout scheme similarly to the results by \citet{janner2019trust}, such that the rollouts are only of length $\horizon \ll \Ti$.

In practice, \opcintmodel cannot be realized as it requires the true (unknown) state transition model~$p$.
However, as we use more on-policy reference trajectories for \opcmodel in \cref{eq:opc_model}, it also converges to zero on-policy error in probability for deterministic policies.
%using an ever-increasing size of reference trajectories $\batchsize$ such that the on-policy error converges to zero in probability.
%
\begin{lemma}
    \label{lem:on_policy_model_error}
    Let $M$ be a \gls{mdp} with dynamics $p(\state_{\ti + 1} \mid \state_\ti, \action_\ti)$ and reward $r < r_{\mathrm{max}}$. Let $\tilde{M}$ be another \gls{mdp} with dynamics $\learnedmodel \neq p$.
    Assume a deterministic policy $\pi: \statespace \mapsto \actionspace$ and a set of trajectories  $\data = \bigcup_{b=1}^{B} \{ ( \refstate^\batch_{\ti}, \refaction^\batch_\ti, \refstate^\batch_{\ti+1} ) \}_{\ti=0}^{\Ti - 1}$ collected from $M$ under $\pi$.
    If we use \ourmethod \cref{eq:opc_model} with data $\data$, then
    \begin{align}
        \lim_{\batchsize \rightarrow \infty} \operatorname{Pr}\left( | \return{} - \modelreturn{}^{\mathrm{opc}} | > \varepsilon \right) = 0 \quad \forall \varepsilon > 0 \quad \text{with convergence rate}  \quad \bigO(1 / \batchsize).
    \end{align}
\end{lemma}
%
We provide a proof in \cref{app:proofs_opc}. \Cref{lem:on_policy_model_error} states that given sufficient reference on-policy data, the performance gap due to model errors becomes arbitrarily small for \emph{any} model \learnedmodel when using \ourmethod.
While the assumption of infinite on-policy data in \cref{lem:on_policy_model_error} is unrealistic for practical applications, we found empirically that \ourmethod drastically reduces the on-policy model error even when the assumptions are violated.
In our implementation, we use stochastic policies as well as trajectories from previous policies, i.e., off-policy data, for the corrections in \ourmethod (see also \cref{sec:exp_continuous_control}).


\subsection{Discussion}
\label{sec:discussion}
\label{sec:limitations}

\paragraph{Epistemic uncertainty}
%
So far, we have only considered aleatoric uncertainty (noise) in our transition models. In practice, modern methods additionally distinguish epistemic uncertainty that arises from having seen limited data \citep{Deisenroth2011PILCO,Chua2018pets}. This leads to a distribution (or an ensemble) of models, where each sample could explain the data. In this setting, we apply $\ourmethod$ by correcting \emph{each sample individually}. This allows us to retain epistemic uncertainty estimates after applying \ourmethod, while the epistemic uncertainty is zero on-policy.

\paragraph{Limitations} Since \ourmethod uses on-policy data, it is inherently limited to local policy optimization where the policy changes slowly over time. As a consequence, it is not suitable for global exploration schemes like the one proposed by \citet{Curi2020hucrl}. Similarly, since \ourmethod uses the observed data and corrects it only with the expected learned model, $\opcmodel$ always uses the on-policy transition noise (aleatoric uncertainty) from the data, even if the model has learned to represent it. While not having to learn a representation for aleatoric uncertainty can be a strength, it limits our approach to environments where the aleatoric uncertainty does not vary significantly with states/actions. It is possible to extend the method to the heteroscedastic noise setting under additional assumptions that enable distinguishing model error from transition noise \citep{schoellig2009optimization}. Lastly, our method applies directly only to \glspl{mdp}, since we rely on state-observations. Extending the ideas to partially observed environments is an interesting direction for future research.


==> figures/tikz/do_not_remove.tex <==
%
